The State of Documentation Practices of Third-party Machine Learning Models and Datasets

Model stores offer third-party ML models and datasets for easy project integration, minimizing coding efforts. One might hope to find detailed specifications of these models and datasets in the documentation, leveraging documentation standards such as model and dataset cards. In this study, we use statistical analysis and hybrid card sorting to assess the state of the practice of documenting model cards and dataset cards in one of the largest model stores in use today--Hugging Face (HF). Our findings show that only 21,902 models (39.62\%) and 1,925 datasets (28.48\%) have documentation. Furthermore, we observe inconsistency in ethics and transparency-related documentation for ML models and datasets.

==> defs.tex <==
\usepackage[english]{babel}
\usepackage[normalem]{ulem}
\usepackage[usenames]{color}
\usepackage{array}
\usepackage{amsmath}
\usepackage{etoolbox}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{comment}
\usepackage{float}
\usepackage{framed}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{multicol}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{soul}
\usepackage{ntheorem}
\usepackage{booktabs, multirow}
\usepackage{subfigure}
\usepackage{url}
\usepackage{changepage,threeparttable}
\usepackage{tabularx,booktabs,ragged2e}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}%
}


\newcommand{\TODO}[1]{\textcolor{blue}{{\it [TODO: #1]}}}

==> figure_imports/RQ1_ModelCard.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/other/RQ1_ModelCard.png}
    \caption{Model Card Example}
    \label{fig:rq1-model-card-example}
\end{figure}

==> figure_imports/RQ1_Steps.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/other/RQ1_Steps.png}
    \caption{RQ1 Steps}
    \label{fig:rq1-steps}
\end{figure}

==> figure_imports/RQ1_WordCloud.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/RQ1/RQ1_WordClouds.pdf}
    \caption{Model Card Content Topics}
    \label{fig:rq1-wordcloud}
\end{figure}

==> figure_imports/RQ2_DatasetCard.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/other/RQ2_Dataset_Card.png}
    \caption{Dataset Card Example}
    \label{fig:rq2-dataset-card-example}
\end{figure}

==> figure_imports/RQ2_DatasetSubsections1.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/RQ2/RQ2_SubsectionCounts1.pdf}
    \caption{Number of Document Dataset Subsections}
    \label{fig:rq2-dataset-subsections}
\end{figure}

==> figure_imports/RQ2_DatasetSubsections2.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/RQ2/RQ2_SubsectionCounts2.pdf}
    \caption{Number of Document Dataset Subsections}
    \label{fig:rq2-dataset-subsections}
\end{figure}

==> figure_imports/RQ2_Steps.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/other/RQ2_Steps.png}
    \caption{RQ2 Steps}
    \label{fig:rq2-steps}
\end{figure}

==> figure_imports/RQ2_WordCloud.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/RQ2/RQ2_WordClouds.pdf}
    \caption{Dataset Card Content Topics}
    \label{fig:rq2-wordcloud}
\end{figure}

==> figure_imports/RQ3_CorePeriphery.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/RQ3/RQ3_FinalGraph.png}
    \caption{Core-Periphery Structure of 214 merged dataset nodes}
    \label{fig:rq3-core-periphery}
\end{figure}

==> figure_imports/RQ3_SimilarityStats.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/RQ3/RQ3_SimilarityHist.pdf}
    \caption{Similarity Score Distributions}
    \label{fig:rq3-similarity}
\end{figure}

==> figure_imports/RQ3_Steps.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/other/RQ3_Steps.png}
    \caption{RQ3 Steps}
    \label{fig:rq3-steps}
\end{figure}

==> sections/3-methods_RQ3.tex <==
\subsection{RQ3 Steps}
\label{sec:methodology:subsec:rq3-steps}

\input{figure_imports/RQ3_Steps}
Figure~\ref{fig:rq3-steps} presents the sequence of steps taken to carry out our analysis for \textbf{RQ3}.

\textbf{Step 3.1} \textit{Dataset Downloading} -- First, we took another random sample of 321 datasets (from the 1,925 datasets with cards) with a confidence level of 95\% and a confidence interval of 5\%. We then proceeded to download that sample of datasets along with all of their "configurations". "Configurations" of a dataset represent the different variants of the dataset uploaded by the dataset owner, for example subsets of the dataset with different sizes or characteristics. Since each of these variants contains one specific view of the dataset, this RQ requires taking a look at all variants. This provided us with 831 archives (1.8 TB in total).

Additionally, many of these datasets (and their configurations) consist of separate training, testing and validation splits, each representing a subset of the entire dataset. These files are provided by Hugging Face as arrow files. For our analysis, we opted to focus on training split files only for two reasons. First, according to the best practices of training machine learning models, the training split of a dataset should be statistically representative in order to avoid troublesome scenarios such as under-fitting and over-fitting~\cite{kelleher_fundamentals_2020}. Second, most models in Hugging Face provide a training split, but not all of them provide a testing and validation split. To obtain a more balanced comparison between datasets, we opted to only use training splits.

\textbf{Step 3.2} \textit{Similarity Calculation} -- Second, we use a digital forensics algorithm called \textit{sdhash} to analyze data similarity between the arrow files~\cite{chow_data_2010}. Sdhash basically takes a file and generates a base-64 encoded string from its binary contents. Then, it compares this string with the strings generated from other files. After these comparisons are made, a score from 1-100 is outputted to denote the significance of the relationship between each pair of files.

We selected \textit{sdhash} because of its robustness in handling large-scale terabyte data in digital forensics investigations, since in our analysis we had to deal with 1.8 TB of data. Furthermore, \textit{sdhash} has been found to outperform its competitors~\cite{chow_data_2010}, and it works equally well on a range of different file types such as text documents, images, audio and video. 

If we consider each configuration of every dataset downloaded in Step 3.1 as a node in a graph, then use the \textit{sdhash} similarity score between every pair of nodes as a weight for the edge between those nodes, the output of Step 3.2 is a dataset similarity graph. However, given that this graph is complete (i.e., each pair of nodes is connected through an edge) and that a given dataset is represented by multiple nodes (i.e., all its configurations), we first need to filter the raw dataset similarity graph before doing any analysis. In particular, we need to (Step 3.3) filter out (configuration) nodes that have too low similarity with other nodes, then (Step 3.4) merge the remaining configuration nodes into one unified dataset node

\textbf{Step 3.3} \textit{Filtering nodes based on similarity threshold} -- In order to determine a threshold for the \textit{sdhash} similarity values we first define $\mathcal{D}=\{d|d \in 321\ studied\ data\ sets\ of\ Step\ 3.1\}$, $conf(d)$ as the set of configurations of a given data set $d \in \mathcal{D}$, $\mathcal{N}_{all}=\{n|  n \in conf(d) \land d \in \mathcal{D}\}$, $\mathcal{E}_{all}=\{\{m,n\}|m \in \mathcal{N}_{all} \land n \in \mathcal{N}_{all} \land m!=n\}$, $edges(n)=\{e|e \in \mathcal{E}_{all} \land n \in e\}$ and $weight(e)$ as the weight of an edge $e \in \mathcal{E}_{all}$. Note that the dataset similarity graph edges in $\mathcal{E}_{all}$ are undirected, hence are represented as sets of 2 nodes. Then, $\forall n \in \mathcal{N}_{all}$, we calculate the average similarity across all edges involving node $n$:

\begin{equation} 
sim_{ind}(n)=\frac{ \sum_{i=1}^{|edges(n)|}{ weight( edges(n)[i] ) } }{|edges(n)|}
\end{equation}

We then created a set of histograms to detect the underlying distributions of the $sim_{ind}$ values to better understand how these scores are behaving. Moreover, we calculated the mean, median, standard deviation, kurtosis and skewness of these distributions to determine how outliers played a role within the datasets. In particular, kurtosis is a measure of whether a distribution is heavy-tailed or light-tailed concerning the normal distribution.  

We obtained a mean $sim_{ind}$ of 43.57 (median 40.30) with a standard deviation of 13.92, a skewness of 1.75 and kurtosis of 2,27. The positive skew of this data meant that most outlier nodes were found towards the right end of the distribution. Hence, based on the histogram we then decided to use the 75th percentile (or 3rd quartile) of 53.87 and rounded to 60, as a similarity threshold to filter out configuration with overall similarity to other nodes.

\textbf{Step 3.4} \textit{Merging configuration with nodes} --
Having filtered out dataset similarity graph nodes with weak $sim_{ind}$ we now move on to merging all remaining configurations of a given dataset into one dataset node. Basically, for each dataset $d \in \mathcal{D}$, we first calculate the average $sim_{ind}(n)$ across all $n \in conf(d) \cap \mathcal{N}_{filtered}$ (i.e., the remaining configurations of $d$), then assign this value to $sim_{merge}(d)$ value to a new graph node for $d$. If no configuration node of $d$ remains after step 3.3, no node is created for $d$. Then, $\forall d' \in \mathcal{D}, d!=d'$ we add an edge $\{d,d'\}$ with as weight the average weight across all possible remaining edges between configurations of d and d', i.e.,  $\{\{n,m\}|n \in conf(d) \cap \mathcal{N}_{filtered} \land m \in conf(d') \cap \mathcal{N}_{filtered}\}$. Finally, we remove all individual configurations nodes $n \in conf(d) \cap \mathcal{N}_{filtered}$, as well as all remaining edges $\mathcal{E}_{all}$. We are left with a filtered dataset similarity graph with the datasets $d \in \mathcal{D}$ as nodes, and a complete set of similarity edges between datasets. Since both the nodes and their edges have changed, we re-calculate $sim_{ind}$ for each dataset node and update their $sim_{merge}$ with these values.

\textbf{Step 3.5} \textit{Stochastic Block Model Visualization} -- Fifth, we model and visualize the filtered dataset similarity graph using stochastic block
modelling to reveal the underlying structures~\cite{holland_stochastic_1983}. This is needed, because the filtered graph is still a complete graph and just shows (average) similarity between each pair of datasets. This does not intuitively allow determining which dataset nodes are the "roots" from which other datasets are derived. Stochastic block modelling identifies communities within larger graphs based on edge (weight) density. We hypothesize that, if some datasets $R$ are more commonly roots from which a larger group of datasets $G$ is derived, $R$ and $G$ would show up as different communities in stochastic block modelling.
We use \textit{graph-tool}~\cite{peixoto_stochastic_2014} to perform stochastic block modelling.

\textbf{Step 3.6} \textit{Dependency Discovery} -- Sixth, we use the stochastic block modelling results to analyze how dataset dependencies obtained through derivation (or even cloning) are reflected within the documentation at Hugging Face. After the analysis of the stochastic block model visualization, we find that the datasets form a core-periphery network, which can be described as "a small number of hubs that gather a disproportionate amount of connections"~\cite{hojman_core_2008}. Armed with this new information we then proceed to check how these relationships might be documented in the corresponding dataset's cards by looking for any mentions of the identified data dependencies.

==> sections/6-rq3-results.tex <==
\section{Dataset Dependency Results (RQ3)}
\label{sec:rq3-results}

\textbf{The mean level of similarity between datasets is approximately 50.6 (out of 100), with 17 (8\%) of the datasets having an average similarity of at least 75 with other datasets}. Table \ref{tab:rq3-sim-score-stats} provides statistical measures such as mean, median, skewness, kurtosis and standard deviation based on the $sim_{ind}$ scores. Moreover, in Figure \ref{fig:rq3-similarity}, a histogram displays the distributions of the similarity scores for the 214 datasets remaining after the merging of the nodes in Step 3.4 in Section \ref{sec:methodology:subsec:rq3-steps}. 

It is readily apparent that the level of similarity is high according to what is specified by \textit{sdhash's} authors who consider anything above 21 (out of 100) high \cite{sdhash_tutorial}. This is hinted at by the mean of 50.58 (compared to the common threshold of 21) \cite{sdhash_tutorial}, with the data spread out substantially according to a standard deviation of 14.28. This distribution is affected by outliers meaning that there are datasets that contain extreme levels of similarity that are influencing the distribution as a whole. This is shown by the kurtosis of 2.27, indicating that the distribution is nearly leptokurtic, i.e., this distribution has a significant number of outliers causing it to be skewed \cite{aggarwal_outliers_2016}. Since the skew is 1.14, then this makes the distribution positively skewed, meaning that the outliers present within this distribution lie rightwards of the mean. 

In other words, there is a clear set of datasets with a disproportionate similarity score and a significant amount of connections within the graph, which is what is referred to as a core-periphery structure \cite{hojman_core_2008}. 

\input{tables/similarity}

\input{figure_imports/RQ3_SimilarityStats}

\textbf{28 datasets represent the roots (pink, gold and blue) of the 214 merged dataset nodes}. Since similarity measures denote correlation, not causation \cite{laundering_an_2017}, we use stochastic block modelling to obtain an approximate idea of which datasets form the roots from which other datasets are derived (copied, customized, etc.). Figure \ref{fig:rq3-core-periphery} displays the visualization of what the core-periphery structure that we identified beforehand looks like with respect to dataset similarity. Due to the complexity of the similarity graphs, even after merging the datasets with their configurations, we show the underlying core-periphery structure in Figure \ref{fig:rq3-core-periphery} without edges.

\input{figure_imports/RQ3_CorePeriphery}

The visualization shows six different groups of nodes. Each color represents a community, of nodes whose edge have comparable distributions of edge weights (i.e., similarity values). For example, the pink, gold, and blue communities in the center are the roots (or cores) of all the other datasets. These cores are the most influential datasets, i.e., the similarity scores of the edges that connect them to other nodes are higher with reference to other communities of nodes. On the other hand, teal, purple and orange nodes are peripheries, meaning that their level of similarity with respect to the edges that connect them to other nodes, is smaller, which is why they surround the cores (edges were elided on the figure).

\textbf{Out of the purple, orange, and teal peripheries 11 (out of 98) purple, 5 (out of 49) orange, and 2 (out of 40) teal datasets document dependencies on core datasets. In addition, 2 blue (out of 6) and 1 gold (out of 12) datasets also refer to another dataset.}

While the exact number of datasets that missed documenting their root datasets is unknown, and would require tedious manual analysis of terabytes of data, the core periphery model seems to suggest that a non-trivial number of datasets on our dataset sample are related (highly similar). The lack of such documentation in most of the datasets studied in this RQ makes it impossible to be aware of and to propagate fixes and updates made to the root datasets. This confirms claims made by previous research, which described these data dependencies as "hidden technical debt" that are also more difficult to detect than regular software dependencies \cite{sculley_hidden_2015}. 

As a first example, the GEM dataset \cite{gem-dataset}, is an important gold core dataset that is used as a benchmark for another 37 datasets \cite{gem-benchmark}, it explicitly documents that e2e\_nlg \cite{e2e-nlg}. A pink core dataset in our sample uses it, and the edge between these two datasets in our filtered dataset similarity graph indeed has a similarity score of 85 marking them as strongly related, demonstrating a dependency between them. 

A counter-example is isixhosa\_ner\_corpus \cite{isixhosa}, a blue core dataset. Its documentation states that it depends on the conll benchmark\cite{conll_web}, a popular benchmark for language datasets. In the datasets that were collected, conll2000 \cite{conll2000} and conll2002 \cite{conll2002} are also present within the pink core nodes. The edges of these two datasets have scores of 83 and 81.5 with ixishosa, showing that there is a dependency between them and that dataset. However, it is difficult to know just what is the nature of this relationship, and which variant was derived from which other dataset. More research is needed to understand how these elements come into play with relation to deployments of datasets.

\begin{framed}
\noindent
\textbf{Summary of RQ3:} The high average \textit{sdhash} similarity of 50.58 in our filtered dataset similarity graph indicates an overall high level of dependencies between datasets, with a limited number of root datasets. Yet those dependencies are not well documented with only  11 (out of 98) purple, 5 (out of 49) orange, and 2 (out of 40) teal nodes of the three peripheries making references to such relationships (in addition to 3 core datasets).
\end{framed}



==> sections/9-conclusion.tex <==
\section{CONCLUSION}
\label{sec:conclusion}

On HF, over 60.38\% of models and 71.52\% of datasets lack any documentation. Even when documentation exists, it often doesn't adhere to HF's Model and Data Card standards~\cite{mcmillan-major_reusable_2021}. Ethical content is notably lacking in the existing documentation.

Our findings suggest a disconnect between user expectations and the current standards, necessitating changes in the current documentation practices and improved tool support to reduce the risk of using third-party datasets and models that lack comprehensive documentation.

==> tables/dataset_card_spec.tex <==
\begin{table}[ht]
\tiny
\centering
\caption{Dataset Card Structure~\cite{mcmillan-major_reusable_2021}}
\resizebox{width=0.4\textwidth}{!}{%
\begin{tabular}{lp{3cm}p{6cm}}
\toprule
\textbf{Section} & \textbf{Subsection} & \textbf{Description}\\
\toprule
\specialcell{Dataset\\Description} & Dataset Summary & This section provides a small description of the datasets\\
\cline{2-3}
 & Supported Tasks and Leaderboards & This section provides an overview of the tasks that a dataset can be used for (i.e. predicting the next word in a sentence). It also provides information about the metrics that are used to measure its performance in a prediction or classification context\\
\hline
\specialcell{Dataset\\Structure} & Data Instances & This describes the different instances that exist within the dataset. Configurations (i.e. datasets with small variations compared to the original) are listed here\\
\cline{2-3}
 & Data Fields & This presents specific information about each feature in a dataset, such as their data type (i.e. int32, float32, string). 
\textbf{Data Splits}: These are the different splits of data that are created for a dataset. In short, this provides the information related to training, test and validation splits for a dataset when applicable\\
\cline{2-3}
 & Data Splits & These are the data splits specified for a dataset. In this section training, test, and validation splits are specified.\\
\hline
\specialcell{Dataset\\Creation} & Curation Rationale (This explains what was done to); & This describes how the dataset was built and for what purposes it is meant to be used\\
\cline{2-3}
 & Initial Data Collection and Normalization & This describes the process of data collection that was done initially and what steps were taken to preprocess the data\\
\cline{2-3}
 & Who are the source language producers? & This describes the groups or entities that were responsible for creating the dataset. For example, if the data was taken from Twitter comments, it would be specified that it was Twitter users that created this data\\
\cline{2-3}
 & Annotations (Annotation Process; Who are the annotators?) & This describes the groups or entities responsible for labeling the data. For instance, if the data came from Twitter, this should explain that the data was created by users from Twitter.    \\
\cline{2-3}
 & Personal and Sensitive Information & This describes any personal or sensitive information that may be present on the dataset\\
\hline
\specialcell{Considerations\\for Using\\the Data} & Social Impact of the Dataset & This outlines any potential impacts that the use of a particular dataset may have when it comes to concerns relating to societal issues\\
\cline{2-3}
 & Discussion of Biases & This lists any potential statistical biases that a dataset may have\\
\cline{2-3}
 & Another Known Limitation & This provides an overview of any other limitations that might potentially exist in the dataset, in addition to the Social Impact and Discussion of Biases sections listed above\\
\hline
\specialcell{Additional\\Information} & Dataset Curators & This is a list of people or organizations that were responsible for curating the data\\
\cline{2-3}
 & Licensing Information & This lists any licensing and legal considerations that a dataset may be subject to\\
\cline{2-3}
 & Citation Information & This provides citation information for a dataset as well as information relating to the origin of a dataset\\
\cline{2-3}
 & Contributions & This lists the people who contributed to the dataset. \\
\bottomrule
\end{tabular}%
}
\label{tab:rq2-dataset-card}
\end{table}

==> tables/dataset_cards_pct.tex <==
\begin{table}[ht]
    \centering
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{|l|l|c|} \toprule
        Type & Number Of Datasets & Percentage(\%) \\\midrule  
        Datasets With Cards & 1,925 & 28.48 \\ 
        Datasets Without Cards & 4,833 & 71,52 \\
        Total & 6,758 & 100 \\
        \bottomrule
    \end{tabular}}
    \caption{Statistics on Datasets with(out) cards}
    \label{tab:rq2-dataset-card-pct}
\end{table}

==> tables/model_card_spec.tex <==
\begin{table}[ht]
\centering
\tiny
\caption{Model Card Structure~\cite{mitchell_model_2019}}
\resizebox{width=0.4\textwidth}{!}{%
\begin{tabular}{lp{3cm}p{6cm}}
\toprule
\textbf{Section} & \textbf{Subsection} & \textbf{Description}\\
\toprule
\specialcell{Model\\Details} & Person or organization developing model &  This provides details about the person or organization that created the model\\
\cline{2-3}
 & Model Date & A specifier that provides the date in which the model was created\\
\cline{2-3}
 & Model Version & A specifier that provides the current version of a model\\
\cline{2-3}
 & Model Type & A specifier that provides the type of model (i.e. neural network, generalized linear model, decision tree, etc.)\\
\cline{2-3}
 & Information about training algorithms, parameters fairness  constraints or other applied approaches and features & This provides a description of how the model was trained and what this process involved\\
\cline{2-3}
 & Paper or other resource for more information & This goes into detail about the resources or papers in which a model was created for\\
\cline{2-3}
 & Citation details & This has information relating to the citation details for a model\\
\cline{2-3}
 & License & This has information about the licensing and legal concerns surrounding a model\\
\cline{2-3}
 & Where to send questions or comments about the model & A point of contact to send inquiries about a model\\
\hline
\specialcell{Intended\\Use} & Primary intended uses & This details the primary tasks for which the model was created for\\
\cline{2-3}
 & Secondary Intended Uses & This details other uses for which the model may apt for, however these are not the ones that the model was specifically created for\\
\cline{2-3}
 & Out-of-scope uses cases & These are specifications of the uses in which the model is not an appropriate choice. Sometimes users may believe that a model is good for a particular case when that may not be true, the purpose of this section is to clarify these confusions and state when these\\
\hline
Factors & Relevant factors & This section refers to factors that are relevant for model performance. The goal here is to specify how performance may vary when considering these\\
\cline{2-3}
 & Evaluation factors & These are the factors that are chosen to be evaluated in terms of performance. This section specifies why these were chosen and establishes further clarification as to why the Evaluation Factors might differ from the Relevant Factors\\
\hline
Metrics & Model performance measures & This specifies which model performance measures are specified. For instance, if accuracy and precision are used, these would be named here\\
\cline{2-3}
 & Decision thresholds & This is a specification that describes the thresholds that might be utilized for the model to make decisions of one type or another\\
\cline{2-3}
 & Variation approaches & This section specifies how uncertainty and variability may be approached. The metrics that may be applied for this section must be specified here. For example, if KL divergence is being used as something to measure uncertainty it would be specified here\\
\hline
\specialcell{Evaluation\\Data} & Datasets & This is an outline of the datasets that are used by a particular model\\
\cline{2-3}
 & Motivation & This section presents the motivation for why the model was created\\
\cline{2-3}
 & Preprocessing & This section specifies the steps that were taken to preprocess the datasets used by the model\\
\hline
\specialcell{Training\\Data} & N/A & This section should ideally specify detailed information about the training data. For instance, it should specify whether the data is proprietary or not. \\
\hline
\specialcell{Quantitative\\Analyses} & Unitary results & This refers to how the model performed in relation to each factor.\\
\cline{2-3}
 & Intersectional results & This states how the model performed concerning the intersection of the evaluated factors. \\
\hline
\specialcell{Ethical\\Considerations} & N/A & This section should explain the ethical considerations that went into the creation of a model.\\
\hline
\specialcell{Caveats and\\Recommendations} & N/A & This section deals with concerns that may not have been addressed in any of the previous sections or that fall outside their scope. \\ 
\bottomrule
\end{tabular}%
}
\label{tab:rq1-model-card}
\end{table}

==> tables/model_cards_pct.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular*}{\linewidth}{p{8em}rr} 
    \toprule
        Type & Number Of Models & Percentage(\%) \\
    \midrule
        Models With Cards & 21,902 & 39.62 \\ 
        Models Without Cards & 33,378 & 60.38 \\
        Total & 55,280 & 100 \\
    \bottomrule
    \end{tabular*}
    \caption{Statistics on Models with(out) cards}
    \label{tab:rq1-model-card-pct}
\end{table}


==> tables/similarity.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|c|c|c|c|c} \toprule
         Distribution & Mean & Median & Std & Skew & Kurt \\ \midrule
         Original & 43.57 & 40.3 & 13.92 & 1.75 & 3.63 \\
         Merged & 50.58 & 49.95 & 14.28 & 1.14 & 2.27 \\
         \bottomrule
    \end{tabular}
    \caption{Similarity Score Statistical Measures}
    \label{tab:rq3-sim-score-stats}
\end{table}
